Correlation between the spatial distribution of the circumstellar disks and the massive stars in the open cluster NGC 6611. Compiled catalog and cluster parameters

Context: the observation of young stars with circumstellar disks suggests that the disks are dissipated, starting from the inner region, by the radiation of the central star and eventually by the formation of rocky planetesimals, over a time scale of several million years. It was also shown that strong UV radiation emitted by nearby massive stars can heat a circumstellar disk up to some thousand degrees, inducing the photoevaporation of the gas. This process strongly reduces the dissipation time scale. Aims: we study whether there exists a correlation between the spatial distribution of stars with circumstellar disks and the position of massive stars with spectral class earlier than B5, in the open cluster NGC 6611. Methods: we created a multiband catalog of the cluster, down to V~23, using optical data from a WFI observation at 2.2m of ESO in the BVI bands, the 2MASS public point source catalog and an archival X-ray observation made with CHANDRA/ACIS. We selected the stars with infrared excess (due to the emission of a circumstellar disk) using suitable color indices independent of extinction, and studied their spatial distribution. Results: the spatial distribution of the stars with K band excess (due to the presence of a circumstellar disk) is anti correlated with that of the massive stars: the disks are more frequent at large distances from these stars. We argue that this is in agreement with the hypothesis that the circumstellar disks are heated by the UV radiation from the massive stars and photoevaporated.

==> multiwave_catalog.tex <==
\section{Optical data reduction}

	In this work we realized a multiband catalog of the region of NGC6611 using optical, near-infrared and X-ray data. The optical data result from the analysis of images in the BVI bands taken with the \textit{Wield Field Camera} (WFI), mounted in the 2.2 meter telescope of the \textit{European Southern Observatory} (ESO) in La Silla (Chile). The near-infrared data, in JHK bands, was taken from the \textit{All-Sky Point Source Catalog} of \textit{Two Micron All-Sky Survey} (2MASS), available on web. The X-ray data come from an observation of 78Ksec with the \textit{ACIS-I} instrument of the CHANDRA satellite. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Instrumental calibration of the optical images}

	The optical images used in this work was taken with WFI the night of 29 July 2000. WFI is a mosaic of $4 \times 2$ CCDs of $2048 \times 4096$ pixels. The angular size of  every pixel is 0.238 arcsec.  The field of view (FOV) of a CCD is then $8.12 \times 16.25$ arcmin, so the total WFI FOV is $33 \times 34$ arcmin. The CCD are separated by intervals of 23.8 arcsec in right ascension and 14.3 arcsec in declination, for a filling factor of 95.5\%.  \par
	The WFI CCDs are characterized by a \textit{Read-Out Noise} equal to 4.5 $e^-/$pixel and a \textit{Gain} equal to 2$e^-/$ADU. \par

	The observations are part of the program ESO Imaging Survey (EIS), including also the PRE-FLAMES program \citep{Mom2001}. Some details of the images analyzed in this work are given in table \ref{tabellaesposizioni}.  The seeing that characterize the exposures is calculated from the FWHM of the profile of the sources observed. The typical seeing for La Silla for optimal observation condition is 1.1 arcsec. In the table \ref{tabellaesposizioni} is evident that the seeing conditions was good during all the night. \par   

\begin{table}[!htb]
\centering
\caption {Characteristic of the observations of NGC6611.}
\vspace{0.5cm}
\begin{tabular}{ccccc}
\hline
\hline
Image& Exposure time(sec) & Time& Filter& Seeing(arcsec) \\
\hline
$NGC6611-1$    &$30 $   &$00:17:02.136$        &$Ic/lwp$       &$1.17$\\
$NGC6611-2$    &$240$   &$00:19:18.375$        &$Ic/lwp$       &$1.31$\\
$NGC6611-3$    &$240$   &$00:25:00.508$        &$Ic/lwp$       &$1.07$\\
$NGC6611-4$    &$30 $   &$00:31:28.294$        &$V/89  $       &$1.43$\\
$NGC6611-5$    &$240$   &$00:33:43.779$        &$V/89  $       &$1.31$\\
$NGC6611-6$    &$240$   &$00:39:21.946$        &$V/89  $       &$1.43$\\
$NGC6611-7$    &$30 $   &$00:46:09.205$        &$B/99  $       &$1.43$\\
$NGC6611-9$    &$30 $   &$01:00:40.413$        &$B/99  $       &$1.07$\\
$NGC6611-10$   &$240$   &$01:02:21.695$        &$B/99  $       &$1.07$\\
$NGC6611-11$   &$240$   &$01:07:40.906$        &$B/99  $       &$1.17$\\
\hline
\hline
\multicolumn{4}{l} {} 
\end{tabular}
\label{tabellaesposizioni}
 \end{table}

	In this work we analyzed 29 images: 10 of NGC6611 (3 with filters V and I, 4 with filter B) and 19 of 3 standard fields necessary for the calibration procedure (see subsect. \ref{calibrazione}). For all the filters there was an exposure of 30 sec and two at least of 240 sec. Figure \ref{wfiI} shows a WFI image in filter I, with evidenced the ACIS FOV. The cluster is in the center of the image.   \par
  
   	\begin*{figure}[!h]
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/6611Ideepmod.ps,width=10cm,angle=0}}
	\caption{WFI image of NGC6611 of 240sec in I band, with evidenced the ACIS FOV, centered on the cluster, and the name of the CCDs of WFI.}
	\label{wfiI}
	\end*{figure}
	
	Before the analysis of the images, it was necessary to apply the IRAF package {\tt MSCRED} for the instrumental calibration of all the images. We used the task {\tt CCDPROC} that allows the \textit{Bias}, \textit{Overscan} and \textit{Flat-Field} correction. For the \textit{Bias} correction were used technical images taken with null exposure time, combined, with the task {\tt ZEROCOMBINE}, in an unique image taking the median value of the counts in the same pixel in the different images. The same procedure was used to combine the \textit{Sky Flat-Field} images (with the task {\tt FLATCOMBINE}), taken at the start of the observation and necessary for the \textit{Flat-Field} correction. \par
	For the images in I band was necessary to remove the \textit{Fringe Pattern}, that is an interference figure created by multiple reflection of the incident radiation inside the semiconductor of the CCD. This was done with the IRAF task {\tt RMVFRINGE} and with a fringe pattern, available on web\footnote{link: http://www.ls.eso.org/lasilla/sciops/2p2/E2p2M/WFI/CalPlan/fringing}, that reproduces the interference figure. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \subsection{Detection of the sources and instrumental magnitude}
   	
	For the detection of the sources recorded in the WFI observations, we used the {\tt DAOPHOT} routine \citep{Stet87}. With the subroutine {\tt FIND} it was possible to detect the sources fitting the observed stellar profile with a gaussian function, whose width depends on the seeing characterizing the frame. It was also necessary to choose a saturation limit, over wich the bright stars saturated the detector; and a significance threshold limit, in unit of the $\sigma$ of the \textit{sky} value of the exposure, under wich faint stars are statistical indistinguishable from noise and average sky brightness. In this case the threshold and saturation limits were set equal to 3.6$\sigma_{sky}$ and 61000$ADU$. \par
	The PSF in the various exposures was determinated by the subroutine {\tt PSF}, fitting a moffattian model for the point-spread function on the stellar profiles. The radius of the region around every star, in which the PSF was defined (parameter \textit{PSF radius}), was set equal to 25-30 pixel, in correspondence with the exposure with better and worse seeing; while the radius of the region in wich the PSF calculated was subtracted to the star's profile, to obtain the position and the magnitude of the star, (parameter \textit{fitting radius}) varied from 5.5 pixels to 7 pixels.    
	With {\tt DAOPHOT} routine we obtained a catalog with star's positions and PSF magnitude for every exposure, and using the routines {\tt DAOMATCH}, {\tt DAOMASTER} and {\tt ALLSTAR} \citep{Stet94} it was possible to correct the difference in position and magnitude of the same star observed in different exposures, dued by shifts and rotations between the images and by the different PSFs characterizing them. \par
	The last routine applied, necessary to calculate the instrumental magnitudes of the stars detected, was {\tt DAOGROW} \citep{Stet90}. The PSF is in fact applied in a region around the stars, limitated by the \textit{fitting radius}, and with this routine it is possible to calculate a correction for the outher part of the stellar profile, that is external to the region delimited by the fitting radius. To do this we adopted the teoric stellar profile given by \citet{King71}, and we used an aperture photometry with radii between 2-24 pixels. The median correction obtained for all the stars detected was -0.008$^m$.    
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \subsection{Calibration of stars' magnitude}
   \label{calibrazione}
	
	For the calibration of the intrumental magnitudes, with NGC6611 were observed 3 standard fields: SA107, SA92 and SA112 \citep{Land92,Stet00}. The standard stars observed covered all the WFI FOV. \par
	The trasformation from the instrumental magnitude system to the standard Johnson-Kron-Cousin one was calculated using the routine {\tt CCDSTD}, the trasformation is then applied to the standard stars by the routine {\tt CCDAVE} and then to all the stars detected by the routine {\tt TRIAL} \citep{Stet05}. \par
	Usually, the typical form of the trasformations used for the calibration is:
	
	\begin{equation}
	\label{banalsolution}
	O_{m} = M_{m} + A_{0} + A_{1} \times{Q} + A_{2}\times{C}
	\end{equation}
	
	where $O_{m}$ is the instrumental magnitudes of the standard stars; $M_{m}$ is the magnitudes of the standard stars in the Johnson-Kron-Cousin system, $A_{0}$ is a magnitude zero-point of the exposure; $A_{1}$ and $A_{2}$ are coefficients that should to be determinated with the zero-point; $Q$ is the airmass of the observation and $C$ is a suitable color. In this case it was necessary to use more complicated forms for the transformations, that were different for the CCDs that compose the WFI mosaic. The general form of the transformations used was:
	
	\begin{equation}
	O_{m} = M_{m} + A_{0} + A_{2} \times{Q} + P_{color} + A_{t} \times{T} + P_{x} + P_{y}
	\label{mysolution}
	\end{equation}
     
     	where $P_{color}$ is a polynomial in the color choosed (at least of second order; the first term was always present); $T$ is the time of the observation and $P_{x}$ and $P_{y}$ are polynomials of the position (at least of third order) of the stars in the CCD (the $x$ axys is in the West-East direction, the $y$ axys in the North-South direction). \par
	It was necessary to use this complicated transformations to correct the different characteristic of the WFI's CCDs, the magnitudes dependence from the position in the WFI mosaic, already studied by several authors (for example \citet{Man01}, \citet{Koch03} and \citet{Corsi03}), and the problem that the standard fields were not observed in a sufficient spanned interval af airmass (from 1.148 to 1.22).\par

	\begin{figure} [!ht]		
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/ccdave_totbansol.ps,width=12cm,angle=0}}
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/ccdave_totsolmia.ps,width=12cm,angle=0}}
	\caption{Difference between the known standard stars' magnitudes in V band and reproduced by the solution (\ref{mysolution}) (upper panel) and the solution (\ref{banalsolution}) (lower panel). It is evident that the use of the solution (\ref{mysolution}) for the calibration improved the error bars and the standard deviation.}
	\label{magsoluzione} 
	\end{figure}

	All the coefficients of the solution (\ref{mysolution}) were calculated fitting the observed and known magnitudes of the standard stars, and then verified with graphs of the residuals of the fit (see later). In figure \ref{magsoluzione} is evident that with the solution (\ref{mysolution}) is possible to improve the error bars and the standard deviation of the distribution. In the other bands the results are analog: the standard deviation with the solution (\ref{banalsolution}) was 0.054 in B band and 0.055 in I band, while with the solution (\ref{mysolution}) the standard deviation obtained were 0.036 in B and 0.029 in I.
	
	\begin{figure} [!h]	
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/nopos.ps,width=12cm,angle=0}}
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/pos.ps,width=12cm,angle=0}}
	\caption{Dependence on a coordinate of the residuals in V band for the standard stars used to calculate the transformations, for two CCD of the WFI mosaic. In the upper panel the standards stars' V magnitudes are reproduced by a transformation without a coordinate polynom, in the lower panel the transformation is comprensive of coordinate polynom.}
	\label{magpos}
	\end{figure}
	

	The effects of the polynomials of CCD's coordinate and colors and the temporal terms are evident in the figures \ref{magpos}, \ref{magcol} and \ref{magtmp}. In the figure \ref{magpos} the spatial dependence on the Y of the V magnitude residuals in the CCD \#52 was removed with a linear and cubic position term, while the spatial dependence on the X in the CCD \#53 was removed using a quadratic and a cubic position term. In the figures \ref{magcol} and \ref{magtmp} is evident as the standard deviation and the median of the residuals of the V magnitudes of the standard stars, in the CCDs \#56 and \#55, improved with a solution comprehensive of color term of second order and temporal term respectively.  
   		

	\begin{figure} [!h]	
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/ccdave_nocol.ps,width=12cm,angle=0}}
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/ccdave_col.ps,width=12cm,angle=0}}
	\caption{Residuals in the V magnitude for the standard stars in the CCD \#56. In the upper panels was used a transformation with a first order ($B-V$) term; in the lower panel a polynomial of the second order. This improved the median and the standard deviation of the distribution.}
	\label{magcol}
	\end{figure}


	\begin{figure} [!h]	
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/ccdave_noT.ps,width=12cm,angle=0}}
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/ccdave_T.ps,width=12cm,angle=0}}
	\caption{Residuals in the V magnitude for the standard stars in the CCD \#55. In the upper panels the V magnitudes are reproduced with a transformation without temporal term; in the lower panel a temporal term was used. It is evident as in the lower panel the standard deviation and the median of the distribution was improved.}
	\label{magtmp}
	\end{figure}
	
	In some case for the calibration of the B magnitudes was necessary to use a term $(B-V)\times Q$ with an empirical determined coefficient equal to -0.016 \citep{Stet05}, to allow for the fact that the radiation in the B band is affected by a more intense exctinction, than the bands with lower frequency, while passing throught the terrestrial atmosphere. \par  
	
	In table \ref{ZP} are reported the zero-points calculated from the solutions (\ref{mysolution}) for the different CCD. It was not possible to calculate the coefficients for the exctinction terms, because of the interval of airmass in the observations of the standard fields, so we were forced to impose them equal to the tyical values for La Silla: 0.14, 0.28 and 0.09 respectively for the V, B and I bands.\par
	
	\begin{table}[!h]
	\centering
	\caption {Magnitude's zero-points for the CCDs of the WFI mosaic, in bands B, V and I, calculated with the transformation (\ref{mysolution}). }
	\vspace{0.5cm}
	\begin{tabular}{cccc}
	\hline
	\hline
	CCD& V  & B  & I  \\
	\hline
	$\#50$ &$0.824$ &$1.01 $  &$1.73 $\\
	$\#51$ &$0.8  $ &$0.561$  &$1.836$\\
	$\#52$ &$1.003$ &$0.637$  &$1.979$\\
	$\#53$ &$0.956$ &$0.639$  &$1.921$\\
	$\#54$ &$0.9  $ &$0.583$  &$1.874$\\
	$\#55$ &$0.9  $ &$0.582$  &$1.889$\\
	$\#56$ &$0.737$ &$0.531$  &$1.763$\\
	$\#57$ &$0.740$ &$0.406$  &$2.442$\\
	\hline
	\hline
	\end{tabular}
	\label{ZP}
 	\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \subsection{Astrometry}
   
   To calculate the celestial coordinates of the stars detected from the CCD's pixel frame, we used the All-Sky Point Source Catalog of Two-Micron All Sky Survey (2MASS) as reference catalog, choosed for its good astrometryc precision \citep{Cutri03}. First, we used the IRAF task {\tt CCXYMATCH} to find a list of common sources between the reference catalog and our one, with a matching tolerance set equal to 0.5 arcsec (parameter \textit{tolerance}). For the identification, the celestial frame of the reference catalog was projected in a plane with the \textit{tanx} projection (a combination of tangent plane projection and polynomials). \par
   The list celestial and pixel coordinate of the common stars was used to find, by a fitting procedure, the transformation between the two reference frames with the task {\tt CCSETWCS}. Then the transformation was applied with the task {\tt SKYPIX} to the catalog of the stars detected to have their celestial coordinate. \par
   The astrometric precision of the optical catalog was obtained matching the optical and the 2MASS catalogs with different matching tolerances (between 0.1 and 2 arcsec). Then we used a statistical procedure that allows to separate the correlated and spurius detection distributions \citep{Damiani04}. The precision at 2$\sigma$ was then equal to 0.6 arcsec.
   
	\begin{figure} [!h]	
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/raggiozoom.ps,width=6cm,angle=0}}
	\caption{Differential distributions of the total, spurious and correlated detections. It is evident that for tolerances larger than 1 arcsec pratically all the detection are spurious.}
	\label{magtmp}
	\end{figure}
      
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \subsection{Comparison with previous catalog}
   
   We compared the photometric and astrometric system of the optical catalog with the only two previous catalogs from CCD about the region of NGC6611: \citet{Hille93} and \citet{Beli99}. The first, consisting of a total of 1026 stars with B, V, J, H and K photometry with a magnitude limit  V$\leq 17^m$, was realized with observations of the Kitt Peak National Observatory (NOAO); the latter is a compilation of previous catalogs, with suitable photometric transformations, comprised the one of \citet{Hille93}, and consist of 2185 stars with the magnitude limit of V$\leq 17^m$. \par
   First, matching thise catalogs with our optical one using a matching tolerance of 2 arcsec, we found sistematic differeces in celestial positions between the common stars: -0.870 in right ascension and +0.177 in declination for the catalog of \citet{Hille93}, and -0.263 in right ascension and -0.674 in declination for the catalog of \citet{Beli99}. After we corrected for this differences, we found the best matching tolerance equal to 0.3 arcsec and 0.5 arcsec for the catalog of \citet{Hille93} and \citet{Beli99} respectively, using the procedure already described. \par
   We have then calculated the difference in magnitude of the common stars, with the results reported in figures \ref{confV} and \ref{confB}. From this figures it is clear that the difference in B band are negligible (the median value is $\leq 0.02^m$), while in V band there is not a good agreement. As already seen, however, the standard stars' magnitudes are well reproduced by the photometric transformations used for the calibration and we will see later that all the optical Color-Magnitude diagrams are autoconsistent. 
   
	\begin{figure} [!h]	
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/magmatch.ps,width=10cm,angle=0}}
	\caption{Difference of the V and B magnitude for the stars common to our optical catalog and the ones of \citet{Hille93} (upper panel) and \citet{Beli99} (lower panel). It is evident that there is not a good agreement between the V magnitudes, while the differences in B band are negligible.}
	\label{confV}
	\end{figure}
   
   From figure \ref{confBH} it is evident that there is not a good agreement between the catalogs of \citet{Hille93} and \citet{Beli99} too.
   
	\begin{figure} [!h]	
	\centerline{\psfig{figure=/home/mguarce/ArticoloNGC6611/magbbelihillmatch.ps,width=7cm,angle=0}}
	\caption{Difference of the B (upper panel) and V (lower panel) magnitudes for the stars common to the catalog of \citet{Hille93} and \citet{Beli99}. The difference in magnitudes are not negligible.}
	\label{confBH}
	\end{figure}

   
   
	

